LENS-GRF: Permutation-Invariant Lesion Evidence Network with Gated Residual Fusion for Acne Severity Grading and Multi-Rater Clinical Oracle Analysis

Localized lesion evidence may improve automated acne severity grading, but detector errors and differences in clinical grading criteria can limit generalization. We evaluated LENS-GRF, a lesion evidence network with permutation-invariant aggregation and gated residual fusion that combines a global Vision Transformer with lesion-region embeddings derived from YOLO11s proposals. Fully automated four-class grading was evaluated on 292 held-out ACNE04 images and, without external adaptation, on 200 PLSBRACNE01 participants represented by 600 facial views. Annotation-assisted inference used registered lesion boxes from three dermatologists in a matched subset of 148 participants. Performance measures included accuracy, macro-averaged precision, sensitivity, and one-versus-rest specificity. Paired comparisons used exact McNemar tests with Holm adjustment. On ACNE04, automated LENS-GRF achieved 80.82% accuracy, 78.80% macro precision, 78.92% sensitivity, and 92.78% specificity. With supplied lesion boxes, internal accuracy averaged 95.89% across three seeds. On the full external cohort, automated LENS-GRF achieved 35.00% accuracy, compared with 42.50% for an independently trained global baseline. External macro precision, sensitivity, and specificity for LENS-GRF were 50.52%, 34.31%, and 78.19%, respectively. In the matched subset, accuracy using Doctor A's lesion annotations was 47.97%, compared with 35.14% for automated inference (unadjusted $p = 0.0094$; Holm-adjusted $p = 0.0846$). Strong internal performance with supplied lesion annotations did not translate into reliable automated grading on the external cohort. More reliable lesion detection, modelling that accounts for differences in grading criteria, and independent validation are needed before clinical use.

==> references_authoryear.tex <==
% MLWA-oriented author-year bibliography for natbib.
% Citation keys unchanged; bibliographic values originate from the author-uploaded file.
% Reference order: first author alphabetical; Lin et al. 2022a/2022b disambiguated.
% Bibliographic metadata require final author verification against publishers.
\begin{thebibliography}{99}

\bibitem[Ardiansyah et~al.(2025)]{lensrwArdiansyah2025}
Ardiansyah, R., Wirarama, I.G.P., Husodo, A.Y.,
Wijayanto, H., Damarjati, C., 2025.
Modification Of YOLOv11n Algorithm Architecture to
Improve Efficiency in Facial Acne Detection,
in: International Conference on Information Technology
and Computing (ICITCOM), 2025, pp. 350--355.
\url{https://doi.org/10.1109/ICITCOM66635.2025.11265682}

\bibitem[Chen et~al.(2025)]{lensintroChen2025}
Chen, Y.-Y., Chan, H.-T., Wang, H.-C., Wang, C.-S.,
Chen, H.-H., Chen, P.-H., Chen, Y.-J., Hsu, S.-H., Hsia, C.-H., 2025.
Feature Feedback-Based Pseudo-Label Learning for
Multi-Standards in Clinical Acne Grading,
Bioengineering 12, 342.
\url{https://doi.org/10.3390/bioengineering12040342}

\bibitem[Gazeau et~al.(2024)]{lensrwGazeauAcneAI}
Gazeau, L., Nguyen, H., Nguyen, Z., Lebedeva, M.,
Nguyen, T., To, T.-D., Le Digabel, J., Filiol, J.,
Josse, G., Perlis, C., Wolfe, J., 2024.
AcneAI: A New Acne Severity Assessment Method Using
Digital Images and Deep Learning,
in: Medical Image Computing and Computer Assisted
Intervention -- MICCAI 2024,
Lecture Notes in Computer Science, vol. 15005,
Springer, 2024, pp. 68--78.
\url{https://doi.org/10.1007/978-3-031-72086-4_7}

\bibitem[Hayashi et~al.(2008)]{lensresultsHayashi2008}
Hayashi, N., Akamatsu, H., Kawashima, M., and Acne Study Group, 2008.
Establishment of grading criteria for acne severity,
\textit{The Journal of Dermatology} 35(5), 255--260.
\url{https://doi.org/10.1111/j.1346-8138.2008.00462.x}

\bibitem[Huynh et~al.(2022)]{lensintroHuynh2022}
Huynh, Q.T., Nguyen, P.H., Le, H.X., Ngo, L.T.,
Trinh, N.-T., Tran, M.T.-T., Nguyen, H.T., Vu, N.T.,
Nguyen, A.T., Suda, K., Tsuji, K., Ishii, T.,
Ngo, T.X., Ngo, H.T., 2022.
Automatic Acne Object Detection and Acne Severity Grading
Using Smartphone Images and Artificial Intelligence,
Diagnostics 12, 1879.
\url{https://doi.org/10.3390/diagnostics12081879}

\bibitem[Ilahi and Gunawan(2025)]{lensrwIlahi2025}
Ilahi, A.F., Gunawan, P.H., 2025.
Optimization Techniques in YOLOv8 for Acne Detection,
in: 12th International Conference on Information Technology,
Computer, and Electrical Engineering (ICITACEE), 2025.
\url{https://doi.org/10.1109/ICITACEE66165.2025.11233019}

\bibitem[Isa and Abu Mangshor(2021)]{lensrwIsa2021}
Isa, N.A.M., Abu Mangshor, N.N., 2021.
Acne Type Recognition for Mobile-Based Application Using YOLO,
Journal of Physics: Conference Series 1962, 012041.
\url{https://doi.org/10.1088/1742-6596/1962/1/012041}

\bibitem[Khairani and Kosala(2025)]{lensrwKhairani2025}
Khairani, N., Kosala, G., 2025.
Acne Detection and Facial Skin Severity Classification
into Four Categories Using You Only Look Once (YOLO) V11,
in: International Seminar on Application for Technology
of Information and Communication (iSemantic),
2025, pp. 554--560.
\url{https://doi.org/10.1109/ISemantic67418.2025.11291986}

\bibitem[Lin et~al.(2022a)]{lensrwLinPrior2022}
Lin, Y., Jiang, J., Chen, D., Ma, Z., Guan, Y.,
Liu, X., You, H., Yang, J., Cheng, X., 2022a.
Acne Severity Grading on Face Images via Extraction
and Guidance of Prior Knowledge,
in: IEEE International Conference on Bioinformatics
and Biomedicine (BIBM), 2022, pp. 1639--1643.
\url{https://doi.org/10.1109/BIBM55620.2022.9995101}

\bibitem[Lin et~al.(2022b)]{lensrwLinKIEGLFN2022}
Lin, Y., Jiang, J., Ma, Z., Chen, D., Guan, Y.,
You, H., Cheng, X., Liu, B., Luo, G., 2022b.
KIEGLFN: A unified acne grading framework on face images,
Computer Methods and Programs in Biomedicine
221, 106911.
\url{https://doi.org/10.1016/j.cmpb.2022.106911}

\bibitem[Lin et~al.(2023)]{lensrwLinDED2023}
Lin, Y., Jiang, J., Chen, D., Ma, Z., Guan, Y.,
Liu, X., You, H., Yang, J., 2023.
DED: Diagnostic Evidence Distillation for acne severity
grading on face images,
Expert Systems with Applications 228, 120312.
\url{https://doi.org/10.1016/j.eswa.2023.120312}

\bibitem[Liu et~al.(2022)]{lensintroLiu2022}
Liu, S., Fan, Y., Duan, M., Wang, Y., Su, G.,
Ren, Y., Huang, L., Zhou, F., 2022.
AcneGrader: An ensemble pruning of the deep learning
base models to grade acne,
Skin Research and Technology 28, 677--688.
\url{https://doi.org/10.1111/srt.13166}

\bibitem[Min et~al.(2021)]{lensrwMin2021}
Min, K., Lee, G.-H., Lee, S.-W., 2021.
ACNet: Mask-Aware Attention with Dynamic Context Enhancement
for Robust Acne Detection,
in: IEEE International Conference on Systems, Man,
and Cybernetics (SMC), 2021.
\url{https://doi.org/10.1109/SMC52423.2021.9659243}

\bibitem[Nainggolan et~al.(2025)]{lensrwNainggolan2025}
Nainggolan, Y.G., Hamami, F., Utama, N.I., 2025.
Inflammatory Acne Detection on Facial Images Using
YOLOv11 with Skin Color Analysis,
in: International Conference on Data Science and Its
Applications (ICoDSA), 2025, pp. 801--806.
\url{https://doi.org/10.1109/ICoDSA67155.2025.11156980}

\bibitem[Prokhorov and Kalinin(2024)]{lensintroProkhorov2024}
Prokhorov, K., Kalinin, A.A., 2024.
Improving Acne Image Grading with Label Distribution Smoothing,
arXiv preprint arXiv:2403.00268v1.

\bibitem[Shaik et~al.(2025)]{lensintroShaik2025}
Shaik, A., Kanichai, J.J., Kurumthottam, A.B.,
Garg, V., Ananthakrishnan, B., 2025.
An experimental evaluation of deep learning-based models
for acne severity classification in humans,
Connection Science 37, 2533867.
\url{https://doi.org/10.1080/09540091.2025.2533867}

\bibitem[Srijiranon et~al.(2026)]{lensintroSrijiranon2026}
Srijiranon, K., Varisthanist, N., Tanantong, T., 2026.
A Study of SimCLR-Based Self-Supervised Learning for
Acne Severity Grading Under Label-Scarce Conditions,
Technologies 14, 116.
\url{https://doi.org/10.3390/technologies14020116}

\bibitem[Traini et~al.(2025)]{lensintroTraini2025}
Traini, D.O., Palmisano, G., Guerriero, C., Peris, K., 2025.
Artificial Intelligence in the Assessment and Grading of Acne
Vulgaris: A Systematic Review,
Journal of Personalized Medicine 15, 238.
\url{https://doi.org/10.3390/jpm15060238}

\bibitem[Trivedi et~al.(2024)]{lensintroTrivedi2024}
Trivedi, N.K., et al., 2024.
Deep Acne: Advancing Automated Acne Identification through
Deep Neural Networks,
in: 2024 1st International Conference on Advanced Computing
and Emerging Technologies (ACET), 2024.
\url{https://doi.org/10.1109/ACET61898.2024.10730442}


% ============================================================
% RELATED WORK REFERENCES [10]--[22]
% ============================================================

\bibitem[Wen et~al.(2022)]{lensintroWen2022}
Wen, H., Yu, W., Wu, Y., Zhao, J., Liu, X.,
Kuang, Z., Fan, R., 2022.
Acne detection and severity evaluation with interpretable
convolutional neural network models,
Technology and Health Care 30, S143--S153.
\url{https://doi.org/10.3233/THC-228014}

\bibitem[Wu et~al.(2019)]{lensrwWu2019}
Wu, X., Wen, N., Liang, J., Lai, Y.-K.,
She, D., Cheng, M.-M., Yang, J., 2019.
Joint Acne Image Grading and Counting via
Label Distribution Learning,
in: Proceedings of the IEEE/CVF International Conference
on Computer Vision (ICCV), 2019, pp. 10641--10650.
\url{https://doi.org/10.1109/ICCV.2019.01074}

\bibitem[Zhang and Ma(2022)]{lensrwZhangMa2022}
Zhang, H., Ma, T., 2022.
Acne Detection by Ensemble Neural Networks,
Sensors 22, 6828.
\url{https://doi.org/10.3390/s22186828}

\bibitem[Zhang et~al.(2024)]{lensrwZhangYOLOv7_2024}
Zhang, D., Jin, C., Zhang, Z., Cao, X., Xue, C., 2024.
Automatic Acne Detection Model Based on Improved YOLOv7,
IEEE Access 12, 194390--194398.
\url{https://doi.org/10.1109/ACCESS.2024.3520641}

\end{thebibliography}


==> references_numbered_BACKUP.tex <==
\begin{thebibliography}{99}

% ============================================================
% INTRODUCTION REFERENCES [1]--[9]
% ============================================================

\bibitem{lensintroTraini2025}
Traini, D.O., Palmisano, G., Guerriero, C., Peris, K.,
Artificial Intelligence in the Assessment and Grading of Acne
Vulgaris: A Systematic Review,
Journal of Personalized Medicine 15 (2025) 238.
\url{https://doi.org/10.3390/jpm15060238}

\bibitem{lensintroChen2025}
Chen, Y.-Y., Chan, H.-T., Wang, H.-C., Wang, C.-S.,
Chen, H.-H., Chen, P.-H., Chen, Y.-J., Hsu, S.-H., Hsia, C.-H.,
Feature Feedback-Based Pseudo-Label Learning for
Multi-Standards in Clinical Acne Grading,
Bioengineering 12 (2025) 342.
\url{https://doi.org/10.3390/bioengineering12040342}

\bibitem{lensintroShaik2025}
Shaik, A., Kanichai, J.J., Kurumthottam, A.B.,
Garg, V., Ananthakrishnan, B.,
An experimental evaluation of deep learning-based models
for acne severity classification in humans,
Connection Science 37 (2025) 2533867.
\url{https://doi.org/10.1080/09540091.2025.2533867}

\bibitem{lensintroLiu2022}
Liu, S., Fan, Y., Duan, M., Wang, Y., Su, G.,
Ren, Y., Huang, L., Zhou, F.,
AcneGrader: An ensemble pruning of the deep learning
base models to grade acne,
Skin Research and Technology 28 (2022) 677--688.
\url{https://doi.org/10.1111/srt.13166}

\bibitem{lensintroSrijiranon2026}
Srijiranon, K., Varisthanist, N., Tanantong, T.,
A Study of SimCLR-Based Self-Supervised Learning for
Acne Severity Grading Under Label-Scarce Conditions,
Technologies 14 (2026) 116.
\url{https://doi.org/10.3390/technologies14020116}

\bibitem{lensintroProkhorov2024}
Prokhorov, K., Kalinin, A.A.,
Improving Acne Image Grading with Label Distribution Smoothing,
arXiv preprint arXiv:2403.00268v1 (2024).

\bibitem{lensintroHuynh2022}
Huynh, Q.T., Nguyen, P.H., Le, H.X., Ngo, L.T.,
Trinh, N.-T., Tran, M.T.-T., Nguyen, H.T., Vu, N.T.,
Nguyen, A.T., Suda, K., Tsuji, K., Ishii, T.,
Ngo, T.X., Ngo, H.T.,
Automatic Acne Object Detection and Acne Severity Grading
Using Smartphone Images and Artificial Intelligence,
Diagnostics 12 (2022) 1879.
\url{https://doi.org/10.3390/diagnostics12081879}

\bibitem{lensintroWen2022}
Wen, H., Yu, W., Wu, Y., Zhao, J., Liu, X.,
Kuang, Z., Fan, R.,
Acne detection and severity evaluation with interpretable
convolutional neural network models,
Technology and Health Care 30 (2022) S143--S153.
\url{https://doi.org/10.3233/THC-228014}

\bibitem{lensintroTrivedi2024}
Trivedi, N.K., et al.,
Deep Acne: Advancing Automated Acne Identification through
Deep Neural Networks,
in: 2024 1st International Conference on Advanced Computing
and Emerging Technologies (ACET), 2024.
\url{https://doi.org/10.1109/ACET61898.2024.10730442}


% ============================================================
% RELATED WORK REFERENCES [10]--[22]
% ============================================================

\bibitem{lensrwWu2019}
Wu, X., Wen, N., Liang, J., Lai, Y.-K.,
She, D., Cheng, M.-M., Yang, J.,
Joint Acne Image Grading and Counting via
Label Distribution Learning,
in: Proceedings of the IEEE/CVF International Conference
on Computer Vision (ICCV), 2019, pp. 10641--10650.
\url{https://doi.org/10.1109/ICCV.2019.01074}

\bibitem{lensrwZhangMa2022}
Zhang, H., Ma, T.,
Acne Detection by Ensemble Neural Networks,
Sensors 22 (2022) 6828.
\url{https://doi.org/10.3390/s22186828}

\bibitem{lensrwLinPrior2022}
Lin, Y., Jiang, J., Chen, D., Ma, Z., Guan, Y.,
Liu, X., You, H., Yang, J., Cheng, X.,
Acne Severity Grading on Face Images via Extraction
and Guidance of Prior Knowledge,
in: IEEE International Conference on Bioinformatics
and Biomedicine (BIBM), 2022, pp. 1639--1643.
\url{https://doi.org/10.1109/BIBM55620.2022.9995101}

\bibitem{lensrwMin2021}
Min, K., Lee, G.-H., Lee, S.-W.,
ACNet: Mask-Aware Attention with Dynamic Context Enhancement
for Robust Acne Detection,
in: IEEE International Conference on Systems, Man,
and Cybernetics (SMC), 2021.
\url{https://doi.org/10.1109/SMC52423.2021.9659243}

\bibitem{lensrwZhangYOLOv7_2024}
Zhang, D., Jin, C., Zhang, Z., Cao, X., Xue, C.,
Automatic Acne Detection Model Based on Improved YOLOv7,
IEEE Access 12 (2024) 194390--194398.
\url{https://doi.org/10.1109/ACCESS.2024.3520641}

\bibitem{lensrwIsa2021}
Isa, N.A.M., Abu Mangshor, N.N.,
Acne Type Recognition for Mobile-Based Application Using YOLO,
Journal of Physics: Conference Series 1962 (2021) 012041.
\url{https://doi.org/10.1088/1742-6596/1962/1/012041}

\bibitem{lensrwIlahi2025}
Ilahi, A.F., Gunawan, P.H.,
Optimization Techniques in YOLOv8 for Acne Detection,
in: 12th International Conference on Information Technology,
Computer, and Electrical Engineering (ICITACEE), 2025.
\url{https://doi.org/10.1109/ICITACEE66165.2025.11233019}

\bibitem{lensrwKhairani2025}
Khairani, N., Kosala, G.,
Acne Detection and Facial Skin Severity Classification
into Four Categories Using You Only Look Once (YOLO) V11,
in: International Seminar on Application for Technology
of Information and Communication (iSemantic),
2025, pp. 554--560.
\url{https://doi.org/10.1109/ISemantic67418.2025.11291986}

\bibitem{lensrwArdiansyah2025}
Ardiansyah, R., Wirarama, I.G.P., Husodo, A.Y.,
Wijayanto, H., Damarjati, C.,
Modification Of YOLOv11n Algorithm Architecture to
Improve Efficiency in Facial Acne Detection,
in: International Conference on Information Technology
and Computing (ICITCOM), 2025, pp. 350--355.
\url{https://doi.org/10.1109/ICITCOM66635.2025.11265682}

\bibitem{lensrwNainggolan2025}
Nainggolan, Y.G., Hamami, F., Utama, N.I.,
Inflammatory Acne Detection on Facial Images Using
YOLOv11 with Skin Color Analysis,
in: International Conference on Data Science and Its
Applications (ICoDSA), 2025, pp. 801--806.
\url{https://doi.org/10.1109/ICoDSA67155.2025.11156980}

\bibitem{lensrwLinKIEGLFN2022}
Lin, Y., Jiang, J., Ma, Z., Chen, D., Guan, Y.,
You, H., Cheng, X., Liu, B., Luo, G.,
KIEGLFN: A unified acne grading framework on face images,
Computer Methods and Programs in Biomedicine
221 (2022) 106911.
\url{https://doi.org/10.1016/j.cmpb.2022.106911}

\bibitem{lensrwLinDED2023}
Lin, Y., Jiang, J., Chen, D., Ma, Z., Guan, Y.,
Liu, X., You, H., Yang, J.,
DED: Diagnostic Evidence Distillation for acne severity
grading on face images,
Expert Systems with Applications 228 (2023) 120312.
\url{https://doi.org/10.1016/j.eswa.2023.120312}

\bibitem{lensrwGazeauAcneAI}
Gazeau, L., Nguyen, H., Nguyen, Z., Lebedeva, M.,
Nguyen, T., To, T.-D., Le Digabel, J., Filiol, J.,
Josse, G., Perlis, C., Wolfe, J.,
AcneAI: A New Acne Severity Assessment Method Using
Digital Images and Deep Learning,
in: Medical Image Computing and Computer Assisted
Intervention -- MICCAI 2024,
Lecture Notes in Computer Science, vol. 15005,
Springer, 2024, pp. 68--78.
\url{https://doi.org/10.1007/978-3-031-72086-4_7}

\bibitem{lensresultsHayashi2008}
Hayashi, N., Akamatsu, H., Kawashima, M., and Acne Study Group,
Establishment of grading criteria for acne severity,
\textit{The Journal of Dermatology} 35(5) (2008) 255--260.
\url{https://doi.org/10.1111/j.1346-8138.2008.00462.x}

\end{thebibliography}

